PoseTrack: A Benchmark for Human Pose Estimation and Tracking

Human poses and motions are important cues for analysis of videos with people and there is strong evidence that representations based on body pose are highly effective for a variety of tasks such as activity recognition, content retrieval and social signal processing. In this work, we aim to further advance the state of the art by establishing "PoseTrack", a new large-scale benchmark for video-based human pose estimation and articulated tracking, and bringing together the community of researchers working on visual human analysis. The benchmark encompasses three competition tracks focusing on i) single-frame multi-person pose estimation, ii) multi-person pose estimation in videos, and iii) multi-person articulated tracking. To facilitate the benchmark and challenge we collect, annotate and release a new %large-scale benchmark dataset that features videos with multiple people labeled with person tracks and articulated pose. A centralized evaluation server is provided to allow participants to evaluate on a held-out test set. We envision that the proposed benchmark will stimulate productive research both by providing a large and representative training dataset as well as providing a platform to objectively evaluate and compare the proposed methods. The benchmark is freely accessible at https://posetrack.net.

==> org.tex <==
% \section*{Workshop Details}
% The workshop will bring together the community of human pose estimation and articulated tracking. The new dataset and benchmark will provide a new means for evaluating and comparing both existing and future methods on pose tracking in a meaningful manner.

%\subsection*{Impact}
\myparagraph{Impact.} After years of extensive research and immense progress on human pose estimation, the research community is now moving towards solving this task in \emph{unconstrained} videos with \emph{multiple} people. As there is no available dataset to meet these criteria to date, our release in conjunction with this workshop will have an immense impact on this research field. Despite possible dangers and pitfalls of benchmarks, previous projects in other related fields, including PASCAL VOC, Middlebury, Sintel, KITTI, and many more, have significantly advanced the state of the art and also allowed for a meaningful analysis of various approaches. We firmly believe that our workshop, together with the new dataset and a centralized benchmark platform, will have a huge impact on the community and will be the first edition of a successful workshop series for the next years.

%\subsection*{Expected outcome}
\myparagraph{Expected outcome.} The main goals of this workshop will be to introduce the dataset and the related challenges, and to discuss the current state of the art as well as future directions to concentrate on. The planned panel discussion with world's leading experts on this problem will be a fruitful input and source of ideas for all participants. As this will be the very first edition in the PoseTrack series, we as organizers also expect to receive valuable feedback from users and from the community on how to improve the benchmark. A few potential issues for the discussion are
\begin{itemize}
\item Where are we in terms of solving the problem of human pose tracking?
\item What are positive and negative points of the PoseTrack dataset?
\item Are current evaluation metrics representative of the solution quality?
\item What are the major failure modes of current methods and how can these be eliminated?
\end{itemize}


% MA: explain why this is going to be a highly visible and well attended workshop
% ...

==> organizers.tex <==
\section*{Appendix B: Biographies of the Organizers}
\label{sec:organizers}
\noindent
{\bf Mykhaylo Andriluka\footnote{Primary contact.}\\ MPI for Informatics, Saarbr\"ucken, Germany}\\
andriluka@mpi-inf.mpg.de\\
%\url{url}\\

\noindent
Mykhaylo Andriluka is a junior research group leader at the Max-Planck Institute for
Informatics. Previously he has been a visiting assistant professor at Stanford University,
post-doctoral researcher at MPII for Informatics, and a visiting researcher at Disney Research
Pittsburgh.  Mykhaylo holds a bachelor degree in applied mathematics from Odessa National
I.I. Mechnikov University, and master's degree in mathematics and PhD degree in computer
science from TU Darmstadt. His research interests are in various aspects of visual human analysis
such as articulated pose estimation and tracking, multi-person tracking, people detection and
activity recognition. Mykhaylos' work has received the best paper awards at AMDO'12 and BMVC'12, and was
a winning entry in the MOTChallenge'16 competition on multi-person tracking. Mykhaylo is also a
co-creator of the popular MPIIHumanPose benchmark for articulated human pose estimation.

\vspace{2em}

%%%%%%%

\noindent
{\bf Umar Iqbal \\ University of Bonn}\\
uiqbal@iai.uni-bonn.de\\
\url{http://umariqbal.info/}\\
Umar Iqbal is a PhD candidate with the Computer Vision Research Group at University of Bonn, Germany. He received his MS degree in Signal Processing from Tampere University of Technology, Finland, in 2013. He worked as computer vision research assistant at Computer Vision Group, COMSATS Institute of Information Technology, Pakistan (2010-2011), Nokia Research Center, Finland (2011-2013), and Tampere University of Technology, Finland (2013). His research interests include human pose estimation, activity recognition, multi-target tracking, and person re-identification. 
\noindent

\vspace{2em}

%%%%%%%

\noindent
{\bf Eldar Insafutdinov\\
MPI for Informatics, Saarb\"ucken, Germany} \\
eldar@mpi-inf.mpg.de\\

\noindent
Eldar Insafutdinov received his Masters degree in Visual Computing from
Saarland University in 2016. Since 2016 he is a PhD student at Max Planck Institute
for Informatics working on articulated human pose estimation and tracking.
He has been serving as a part of organizing committee for several
Computer Vision conferences.


\vspace{2em}

%%%%%%%

\noindent
{\bf Anton Milan\\ Australian Centre for Visual Technology, University of Adelaide}\\
anton.milan@adelaide.edu.au\\
\url{http://research.milanton.net}\\

\noindent
Anton Milan (n\'{e} Andriyenko)
received his Diplom degree in Computer Science
(Dipl.-Inform.) from the University of Bonn in 2008 and his PhD from the  Technische Universit\"at Darmstadt in 2013. 
He has worked as a software developer in the computer graphics industry and currently holds his position as a post-doctoral fellow at the University of Adelaide in Australia.
He served as a reviewer for various computer vision conferences and journals.
His research interests include robotic vision, multiple people tracking and pose estimation and machine learning. He co-authored the MOTChallenge benchmark and has co-organized three workshops on benchmarking multi-target tracking (WACV 2015, ECCV 2016 and CVPR 2017 (upcoming)).

\vspace{2em}

%%%%%% 

\noindent
{\bf Leonid Pishchulin \\ MPI for Informatics, Saarbr\"ucken, Germany}\\
leonid@mpi-inf.mpg.de\\

\noindent
Leonid Pishchulin received his Masters degree in Computer Science from
RWTH Aachen University in 2010 and his PhD from Max Planck Institute
for Informatics in 2016. Since 2015 he is a research scientist in
computer vision industry. He has been serving as a part of organizing
committee for multiple top-tier conferences and journals. His research
interests are articulated human pose estimation and tracking, 3D human
body shape and motion analysis, and human activity recognition.

\vspace{2em}
 
 
%%%%%%%

\noindent
{\bf Juergen Gall\\ University of Bonn}\\
gall@iai.uni-bonn.de\\
\url{https://pages.iai.uni-bonn.de/gall_juergen/}\\

\noindent
Juergen Gall obtained his B.Sc. and his Master’s degree in mathematics from the University of Wales Swansea (2004) and from the University of Mannheim (2005). In 2009, he obtained a Ph.D. in computer science from the Saarland University and the Max Planck Institut f{\"u}r Informatik. He was a postdoctoral researcher at the Computer Vision Laboratory, ETH Zurich, from 2009 until 2012 and senior research scientist at the Max Planck Institute for Intelligent Systems in T\"ubingen from 2012 until 2013. Since 2013, he is professor at the University of Bonn and head of the Computer Vision Group. He co-organized several work-shops and tutorials on solving real-world vision problems with RGB-D cameras and on affordances for scene analysis in conjunction with CVPR/ICCV/ECCV/RSS. He served as area chair for ECCV and ICCV in 2015 and 2016 and was program chair for the German Conference on Pattern Recognition in 2015.
% He co-organized several workshops and tutorials on solving real-world vision problems with RGB-D cameras and on affordances for scene analysis. He received a grant for an Emmy Noether research group from the German Research Foundation (DFG) in 2013 and the German Pattern Recognition Award of the German Association for Pattern Recognition (DAGM) in 2014.
\vspace{2em}

%%%%%%%

\noindent
{\bf Bernt Schiele\\ MPI for Informatics, Saarbr\"ucken, Germany}\\
schiele@mpi-inf.mpg.de\\
% \url{https://www.mpi-inf.mpg.de/departments/computer-vision-and-multimodal-computing/people/bernt-schiele/}\\

\noindent
Bernt Schiele is Max-Planck-Director at MPI Informatics and Professor at Saarland University since 2010.
He studied computer science at the University of Karlsruhe, Germany. He worked on his master thesis in the field of robotics in Grenoble, France, where he also obtained the ``diplome d'etudes approfondies d'informatique''. In 1994 he worked in the field of multi-modal human-computer interfaces at Carnegie Mellon University, Pittsburgh, PA, USA in the group of Alex Waibel. In 1997 he obtained his PhD from INP Grenoble, France under the supervision of Prof. James L. Crowley in the field of computer vision. The title of his thesis was ``Object Recognition using Multidimensional Receptive Field Histograms''. Between 1997 and 2000 he was postdoctoral associate and Visiting Assistant Professor with the group of Prof. Alex Pentland at the Media Laboratory of the Massachusetts Institute of Technology, Cambridge, MA, USA. From 1999 until 2004 he was Assistant Professor at the Swiss Federal Institute of Technology in Zurich (ETH Zurich). Between 2004 and 2010 he was Full Professor at the computer science department of TU Darmstadt.

%%%%%%%


==> table_per_frame_ap_test.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c c ccc ccc c c@{}}
    \toprule
    Model& Training Set & Head   & Sho  & Elb & Wri & Hip & Knee & Ank & mAP \\
    %&  &  & & & & & & & CNN & infer.\\
    \midrule
     Top-Down & MPII + our dataset & 75.3 & 72.3 & 67.1 & 60.0 & 63.3 & 61.5 & 56.1 & 65.1 \\ 
     %\midrule
    \bottomrule
  \end{tabular}
% \vspace{0.75em}
\caption[]{Results of baseline models on the task of per-frame multi-person pose estimation (mAP). Test set.
}
\label{tab:per-frame-ap-test}
%  \vspace{-1.5em}
\end{table}


==> table_stats.tex <==

\tabcolsep 6pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{l c c c}
    \toprule
    & num. poses & num. tracks & num. videos  \\
    \midrule
 Training &  61178 &  2437 & 292\\
Validation & 18996 & 695 & 50 \\
Test & 73471 & 2334 & 208 \\
\midrule
Total & \textbf{153615} & \textbf{5446} & \textbf{550} \\
    \bottomrule
  \end{tabular}
\caption[]{Statistics of the train/val/test splits of our dataset.}
\label{tab:dataset_stats}
%  \vspace{-2.5em}
    \vspace{-0.3cm} 
\end{table}





==> table_tracking_mota_test.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} c c ccc ccc c | c c@{}}
    \toprule
    Model& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & Total & mAP \\
    %&  &  & & & & & & & CNN & infer.\\
    \midrule
     ArtTrack & 58.6 & 56.8 & 47.9 & 41.0 & 47.6 & 45.2 & 39.6 & 48.1 & 59.4\\ 

%\midrule
    \bottomrule
  \end{tabular}
% \vspace{0.75em}
\caption[]{Results of the baseline tracking models on the task of multi-person pose tracking (MOT). Test set.
}
\label{tab:tracking-mota-test}
%  \vspace{-1.5em}
\end{table}

